Gradient Shaping: Enhancing Backdoor Attack Against Reverse Engineering

Most existing methods to detect backdoored machine learning (ML) models take one of the two approaches: trigger inversion (aka. reverse engineer) and weight analysis (aka. model diagnosis). In particular, the gradient-based trigger inversion is considered to be among the most effective backdoor detection techniques, as evidenced by the TrojAI competition, Trojan Detection Challenge and backdoorBench. However, little has been done to understand why this technique works so well and, more importantly, whether it raises the bar to the backdoor attack. In this paper, we report the first attempt to answer this question by analyzing the change rate of the backdoored model around its trigger-carrying inputs. Our study shows that existing attacks tend to inject the backdoor characterized by a low change rate around trigger-carrying inputs, which are easy to capture by gradient-based trigger inversion. In the meantime, we found that the low change rate is not necessary for a backdoor attack to succeed: we design a new attack enhancement called \textit{Gradient Shaping} (GRASP), which follows the opposite direction of adversarial training to reduce the change rate of a backdoored model with regard to the trigger, without undermining its backdoor effect. Also, we provide a theoretic analysis to explain the effectiveness of this new technique and the fundamental weakness of gradient-based trigger inversion. Finally, we perform both theoretical and experimental analysis, showing that the GRASP enhancement does not reduce the effectiveness of the stealthy attacks against the backdoor detection methods based on weight analysis, as well as other backdoor mitigation methods without using detection.

==> 1-intro.tex <==
\section{Introduction}\label{sec:intro}
\vspace{-0.3cm}
Critical to trustworthy AI is the trustworthiness of machine learning (ML) models, which can be compromised by malevolent model trainers, evil-minded training data providers, or any parties with access to any link on the ML supply chain (e.g., pre-trained models) to inject a backdoor (aka., trojan). A backdoored model is characterized by strategic misclassification of the input carrying a unique pattern called \textit{trigger}: e.g., special glasses worn by a masquerader to impersonate an authorized party against a compromised facial-recognition system. So the assurance of ML models can only be upheld by effectively detecting those backdoored models, which have been intensively studied in recent years. Existing backdoor defense methods have been reviewed by an SoK paper~\cite{backdoorsurvey}: among seven general defense strategies, two are based on backdoor detection, which uses either the trigger inversion (aka. trigger synthesis) or weight analysis techniques (aka. model diagnosis)~\cite{NC}\cite{abs}\cite{k-arm}\cite{AC}\cite{MNTD}. The most concrete progress in the backdoor detection has been at least partially attributed to \textit{trigger inversion} related techniques, as evidenced in the TrojAI competition~\cite{trojai} (9 out of 11 rounds won by inversion approaches, the rest two won by weight analysis) and the BackdoorBench project~\cite{dbd-backdoor-defense-iclr2022} (leading performers are mostly gradient-based trigger inversion). However, little has been done to understand whether these approaches raise the bar to the backdoor attacks or are just another porous defense line permeable by the knowledgeable adversary.

% \ma{Maybe remove the discussion of weight analysis here?}
% Added in Intro

\vspace{2pt}\noindent\textbf{Achilles' heel of gradient-based optimization}. Trigger inversion is a technique that automatically recovers a pattern causing an ML model to misclassify the pattern-carrying input. Such a pattern is considered a putative trigger and utilized to determine whether the model is indeed backdoored. This reverse-engineering step mostly relies on gradient descent, which seeks the greatest tendency towards misclassification following the opposite direction of the model's gradient with regard to its input. A prior study shows that almost all proposed trigger inversion approaches are gradient-based~\cite{backdoorsurvey}. Although gradient-based optimization can converge to a local optimum, this convergence is contingent upon selecting a proper size for each search step and a proper initialization. In the presence of a function with low robustness around trigger-inserted inputs (e.g., the one having a steep slope (large changing rate), as shown in Figure~\ref{fig:hole}), a large step size could overshoot the local minimum for the trigger that leads to misclassification. On the other hand, a small step size could render the convergence process exceedingly slow and increase the probability that the optimizer converges to another local minimum, practically thwarting any trigger inversion attempt. 
% On the other hand, another major backdoor detection technique, weight analysis, is a technique that utilizes a classifier to distinguish the Trojan model. Such a classifier takes the parameters of the victim model as input and outputs the likelihood of the existence of a backdoor. This kind of classifier relies on observing multiple times of behavior of the Trojan model and benign model parameters within the same task. Then summarize a strong signal from model parameters or, even more intuitively, train a classifier on sets of parameters, then utilize the  summarized signal or trained classifier to distinguish the Trojan model. When a function with low robustness around trigger-inserted inputs indicates more area has been predicted correctly in the local area around trigger-inserted inputs, and for a benign model, this lead to a function with low robustness around trigger-inserted inputs could hardly be detected by weight analysis because almost the entire local area around trigger-inserted inputs should be predicted correctly. This leads to a low trigger robustness model being more similar to a benign model.
So a fundamental question not asked before is why gradient-based reverse engineering works so well on the backdoors injected using today's techniques and whether a more powerful backdoor capable of defeating the inversion can be injected under practical threat models.



\vspace{2pt}\noindent\textbf{Analysis and findings}. To answer this question, we conducted the first study to understand the limitations of trigger inversion. Our research shows that today's backdoor injection techniques, both loss-function manipulation, and data poisoning, turn out to be quite amenable to gradient-based optimization. Actually, given the relatively simple features that characterize today's triggers (e.g., geometric shapes), a backdoor learned could be more robust to the noise added to its trigger than the benign task the infected model claims to perform, as observed in our experiments:  we found that oftentimes, backdoors tend to be more resilient to the noise than the primary task to the perturbation on its features (Section~\ref{sec:observation}).

This observation indicates that the backdoor can be invoked by not only the trigger but a wide range of its variations. Therefore, the average change rate of the backdoored model around trigger-inserted inputs for recognizing a trigger cannot be too high, which can be easily captured with a relatively larger scope of  search step size and initialization selection. This explains why trigger inversion works so well in backdoor detection. However, a slow change rate (or high trigger robustness) is \textit{not} required for a backdoor attack to succeed. Our research shows that the change rate can be increased through data contamination without undermining the effectiveness of the backdoor attack. In our research, we designed a simple algorithm that could enhance the backdoor attack, called gradient shaping (\ourmethod{}) that utilizes both mislabeled data and correctly labeled data with noised triggers to contaminate the training set, in an opposite way to the adversarial training~\cite{adversarialtraining}, so as to narrow down the variation of the trigger pattern capable of invoking the backdoor. We theoretically analyze this approach and show that it effectively raises the change rate, thereby weakening the detection ability from trigger inversion.


It is worth noting that \ourmethod{} represents a different type of backdoor attack compared with the stealthy backdoors proposed recently (e.g., \cite{lira} \cite{ren2021simtrojan}). Existing stealthy backdoor methods attempt to devise specific triggers, often dependent on the target neural network model so that they are hard to detect and mitigate by defense methods. \ourmethod{}, on the other hand, is a generic trigger injection method that injects any trigger designed by the attacker into a target model so that the trigger is harder to detect and mitigate by the trigger inversion-based backdoor defenses. As a result, \ourmethod{} can be combined with existing stealthy backdoor methods to enhance their capability to evade the trigger inversion-based defenses. 
Our studies show that existing backdoor attacks less capable of evading trigger inversion can be boosted by \ourmethod{} to easily defeat most representative inversion protection, including Neural Cleanse (NC)~\cite{NC}, tabor~\cite{tabor}, k-arm~\cite{k-arm}, pixel~\cite{pixelbackdoor}, rendering them incapable of capturing any trigger of a backdoored model.  

We also perform a theoretical and experimental analysis (Section \ref{sec:theory}) to show that \ourmethod{} does not make the backdoor more vulnerable to weight analysis, which is the other mainstream technique for backdoor detection. In particular, our experiment shows that the \ourmethod{} enhancement does not decrease the effectiveness of the backdoor attacks such as DFST~\cite{DFST}, AB~\cite{adaptive-blend}, and DEFEAT~\cite{defeat} against the weight analysis-based detection. Finally, our study demonstrates that the effectiveness of \ourmethod{} against trigger inversion does not make the enhanced attacks more vulnerable to other backdoor mitigation or unlearning techniques, such as Fine-purning~\cite{fine-purning}, NAD~\cite{NAD}, Gangsweep~\cite{zhu2020gangsweep}, DBD~\cite{DBD}, and RAB~\cite{rab}. 

\vspace{2pt}\noindent\textbf{Contributions}. The contributions of the paper are outlined below: 

\vspace{2pt}\noindent$\bullet$\textit{ First in-depth analysis on trigger inversion}. We report the first in-depth analysis that explains why trigger inversion works so well on backdoor detection. This leads to the discovery of the fragility of the advance we made in this area, given the observation that the weakness of today's trigger injection can be addressed without undermining the effectiveness of the backdoor. 

\vspace{2pt}\noindent$\bullet$\textit{ New backdoor injection technique}. Our new understanding of trigger inversion has been made possible by a new backdoor injection technique, which exploits the fundamental limitation of gradient-based optimization and works under realistic threat models. As such, this method can enhance existing backdoor attacks, making it more effective in evading trigger inversion, but not less effective in evading the weight analysis-based detection and other defenses.
\vspace{-0.3cm}













==> 10-Discussion.tex <==
\section{Discussion}\label{sec:Discussion}

The magnitude of the additive noise introduced by \ourmethod{} is controlled through the parameter $c$. As explained in Section~\ref{subsec: Gradient Shaping}, the noise added to a trigger weakens its robustness. The smaller the magnitude (controlled by $c$) of the noise is, the less robust the trigger is. We study the effect of $c$ on the trigger and backdoored models in Appendix~\ref{subsec: White noise}. We observe that with the increase of the noise level $c$, the trigger robustness increases, so as the detection effectiveness of NC. This echoes our observation in Section~\ref{sec:observation} that the detection performance positively correlates with trigger robustness. However, existing inversion-based detection methods are less effective against \ourmethod{} enhanced attacks as the detection performance is low under different noise levels. When the noise level is very low, the model accuracy and the attack success rate slightly degrade, because a very small $c$ makes the trigger robustness degrade below that of the primary task of the target model. When this occurs, \ourmethod{} is subjected to the backdoor mitigation such as RAB~\cite{rab} that nullifies the effect of the trigger. Please see more discussions in Appendix (\ref{subsec: White noise}).


==> 11-related-work.tex <==
\section{Related Work}
In literature, many backdoor attacks aim to make the backdoor more stealthy. For data contaminating backdoor attacks, most recent works are focused on utilizing generative models and/or data-specific information to enhance the backdoor stealthiness~\cite{ren2021simtrojan}~\cite{wang2022bppattack}~\cite{qi2022circumventing}. To minimize the difference in the feature representations between trigger-inserted input (with the target label) and the corresponding benign input (with the source label).
Moreover, many researches focused on generating adaptive triggers. For example,~\cite{feng2022stealthy} employed a backdoor generation network to generate an invisible backdoor pattern for specific input. 
On the other hand, many studies are focused on contaminating datasets by clean label data~\cite{ning2021invisible}~\cite{doan2021backdoor}~\cite{zeng2022narcissus} to evade the manual dataset reviews.

\label{sec:related work}

==> 12-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we studied why the trigger inversion algorithms are so effective on backdoor defense and found that it is because the current backdoor attacks inject the triggers more robust to the noise and thus can be easily reconstructed by gradient-based trigger inversion algorithms. Based on this analysis, we proposed a gradient shaping (GRASP) approach to enhancing backdoor attacks, which reduces the robustness of the injected trigger through  data poisoning to evade the backdoor defense using trigger inversion algorithms. We conducted both theoretical and experimental analyses to show that \ourmethod{} enhanced the effectiveness of state-of-the-art stealthy backdoor attacks against trigger inversion algorithms while does not reduce their effectiveness against the other backdoor defense, including those based on weight analysis.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> 5-theory.tex <==

\section{Theoretical Analysis of \ourmethod{}}\label{sec:theory}


In this section, we present the theoretical analysis of \ourmethod{} to answer two questions: 1) why gradient-based trigger inversion methods are effective on the triggers with high robustness; and 2) % Secondly, base on the analysis from the first question, we analysis that 
why \ourmethod{} can render trigger inversion ineffective, even though these techniques perform exceedingly well on existing backdoor attacks. More specifically, in section~\ref{subsec:3 condition}, we attempt to bridge the relationship between trigger robustness and the efficiency of gradient-based trigger inversion methods. Because the theoretical analyses for the optimization of a generic target function (approximated by a deep neural network) are very challenging, our analysis is focused on the optimization of three types of functions, each under different constraints.

First, when we approximate our target high-dimensional function by a convex relaxation that Lemma~\ref{Lemma:borrowed_SGD convergence} borrowed from~\cite{convexthm}, shows that the convergence of the gradient-based optimizations are faster when the function has lower Lipschitz constant. Because a convex function with the low Lipschitz constant around the trigger-inserted points indicates the high robustness of the trigger (Theorem \ref{thm:trojan_increaseing_rate_function_lipschitz}), our analysis explains the good performance of the gradient-based trigger inversion methods on the triggers with high robustness.

Second, when the target function is a one-dimensional non-convex piece-wise linear function, which is one of the most regular types of neural network function (such as neural network with ReLU activation function), we prove in Theorem~\ref{thm:MC_proof} that the probability that the gradient descent algorithm converges to the desired optimum (i.e., the trigger-inserted point) is greater when the convex hull is larger. Because the larger convex hull around the trigger-inserted points indicates the higher robustness of the trigger, our analysis explains the good performance of the gradient-based trigger inversion methods on the robust triggers under this condition.

Finally, when the target function is high dimensional non-convex but satisfies the PL condition~\cite{PL_condition}, we prove in Theorem \ref{thm:PL_condition} that the gradient-based optimization algorithms converge faster to the desirable optimum (i.e., the trigger-inserted point) if the local Lipschitz constant near the optimum is lower. As shown in recent research \cite{terjek2019adversarial,krishnan2020lipschitz}, the neural network with high robustness tends to have a lower Lipschitz constant, our analyses again showed the high correlation between the trigger robustness and the efficiency of the gradient-based trigger inversion methods.


Next in section~\ref{subsec: why Grasp can render}, we attempt to answer the second question: by proving Theorem \ref{thm1a}, we showed that when using \ourmethod{} to inject a trigger, the backdoored model will have greater local Lipschitz constant around the trigger-inserted points, thus reducing the robustness of the backdoor, which can render trigger inversion ineffective.

\subsection{Why Inversion Works on Robust Triggers} \label{subsec:3 condition}


%\subsection{Why trigger inversion works well on high trigger robustness} \label{subsec:3 condition}

\noindent Before we elaborate our theorem, we need to first formally define some concepts and a Lemma from \cite{yang2020adversarial}: 

\begin{definitionbold}[Astuteness]
A classifier $f: \mathcal{X} \rightarrow \mathcal{Y}$ is {\em astute} at an input sample $x$, if the predicted label by $f$ is the same as the true label: $\hat{y}=z(f(x))=y$. 

\end{definitionbold}
\begin{definitionbold}[r-local minimum]
A function $f: \mathcal{X} \rightarrow \mathbb{R}$ has a (unique) $r$-local minimum at $x^{\star}$, if there is no other $x$ on which $f$ gets lower or equal value than what can get on $x^*$, within the ball centered on $x^*$ with radius $r$, 
i.e., $f(x) > f(x^*), \forall x, \|x-x^*\|_2 \leq r$.
%i.e., $||x - x^{\star}|| \leq r$.

\end{definitionbold}
\begin{definitionbold}[Increasing rate and relaxation function]
Given a function $f: \mathcal{X} \rightarrow \mathbb{R}$ with a $r$-local minimum at $x^{\star}$, we define that $f$ has an increasing rate of $\kappa$ at $x^{\star}$, if there exists some $\kappa \geq 0$ and $c_{\kappa} \geq 0$, such that
$f(x) - f\left(x^{\star}\right) \geq \sup_{c_{\kappa},\kappa} c_{\kappa} \cdot\left\|x-x^{\star}\right\|_{2}^{\kappa}$, when $\|x -x^{\star}\| \leq r$. Accordingly, we refer the function $\bar{g}(x) = c_{\kappa} \cdot\left\|x-x^{\star}\right\|_{2}^{\kappa}$ as the relaxation function of $f$ at $x$. 
\end{definitionbold}

\begin{definitionbold}[Local Lipschitz constant]
For a function $f: \mathcal{X} \rightarrow \mathcal{Y}$, a given input $x$ and a pre-defined radius $r$, if $L(f,\mathcal{X}_{x,r})$ exists and is finite, where $\mathcal{X}_{x,r} = \{x':\|x'-x\|_2 < r\}$ and
\begin{equation}
\begin{array}{r@{\quad}l}
 L(f,\mathcal{X}_{x,r}) = \sup_{x_1,x_2 \in \mathcal{X}_{x,r}} \frac{||f(x_2) - f(x_1)||_2}{||x_2-x_1||_2},
\end{array}
\end{equation}
we define $L(f,\mathcal{X}_{x,r})$ as the local Lipschitz constant of $x$ with radius $r$ for function $f$.
\end{definitionbold}

\begin{lemmabold}
Consider the data distribution $X$, and assume the minimum $l_2$ norm between any two different class data is $r$. If a function is astuteness in $X$, then $f$ has a local Lipschitz constant of $r'$ around any $x \in X$ such that $r'\geq r$ 
\end{lemmabold}


Fig.~\ref{fig:increasingrate} illustrates the concept of the increase rate by using three one-dimensional functions with $c = 1, \kappa = 0.5$, $1$, and $2$, respectively, at the $r$-local minimum $x^{\star}$. Note that, in the first two conditions, we consider the optimization within the trigger area, which means that we assume the trigger area is known, so we only need to consider the first term in the Eq~\ref{formula: ori opt}. In the third condition, we do not have such an assumption; we consider both terms in Eq~\ref{formula: ori opt}. 


% \begin{figure}[htbp]
% %\ref{fig:increasingrate}
% \captionsetup{font=small}
% \subfloat[$\kappa = 0.5$]{\includegraphics[height=0.75in]{images/kappa=0.5.jpeg}}
% \enspace
% \subfloat[$\kappa = 1$]{\includegraphics[height=0.75in]{images/kappa=1.jpeg}}
% \enspace
% \subfloat[$\kappa = 2$]{\includegraphics[height=0.75in]{images/kappa=2.jpeg}}
% \vspace{0cm}
% \caption{The schematic illustration of three one-dimensional functions with the increasing rates of $\kappa = 0.5$, $1$, and $2$, respectively at an $r$-local minimum $x^{\star}$. Here, the original function is shown in black while the relaxation function is in yellow.}
% \label{fig:increasingrate} 
% \end{figure}



We attempt to connect the local Lipschitz constant of the target function used by trigger inversion with the increasing rate of the relaxation function near the trigger-inserted data point so that later we can exploit the Lipschitz constant of the relaxation function for the convergence analysis of the gradient-based trigger inversion.   


\begin{theorembold}
\label{thm:trojan_increaseing_rate_function_lipschitz}
Consider a function $f:\mathcal{X} \rightarrow \mathbb{R}$ that has a unique $r$-local minimum around $x^*$, i.e., 
$\forall x \in \mathcal{B}= \{x: \|x - x^*\| < r\}, f(x^*) < f(x)$ holds. 
Assuming the increasing rate of $f(x)$ is $\kappa$ at $x$. If $\kappa < 1, c_{\kappa} > 1$, for any $x$ satisfies $\|x - x^*\|_2 > 1$, we have:
\begin{equation}
    L(f, \mathcal{X}) \geq c_{\kappa}\left\|x_{1}-x_{2}\right\|_{2}^{k-1}
\end{equation}

\noindent where $x_1,x_2\in \mathcal{X}$, and $L(f, \mathcal{X})$ is the local Lipschitz constant of $f(x)$ at $x$.
\end{theorembold}


The proof of Theorem \ref{thm:trojan_increaseing_rate_function_lipschitz} is given in 13.4 of the online document~\cite{online_document}. Theorem \ref{thm:trojan_increaseing_rate_function_lipschitz} studies a local sphere region with the center at an optimum point (i.e., the trigger-inserted sample) and the radium as the distance between the center and the initial point (typically a clean sample) of the optimization, and relaxes the target function used by trigger inversion into a convex function (i.e., the {\em relaxation function}) within the local sphere region, so that the Lipschitz constant of the relaxation function can be used to approximate the local Lipschitz constant of the original target function.
Here, the relaxation is used as a tool to study the convergence of gradient-based optimization on a non-convex function like the target function in Eq.\ref{formula: ori opt}.
Even though the relaxation may not resemble the target function, it approximates an essential property (i.e., the local Lipschitz constant) of the target function near the optimum point. 

Finally, as shown Lemma~\ref{Lemma:borrowed_SGD convergence}, which is borrowed from \cite{convexthm}, the gradient-based optimization algorithms, including  the three most commonly used optimizers in deep learning: stochastic gradient descent (SGD), projected gradient descent (PGD), and the accelerate gradient descent (AGD), converge more slowly to a local optimum of a convex function when the change rate (i.e., the Lipschitz constant) of the function is greater. 

\begin{lemmabold} \label{Lemma:borrowed_SGD convergence}
For a convex function $f:\mathcal{X} \rightarrow \mathcal{Y}$, If $g(x)$ is the sub-gradient set of $f$ at $x \in \mathcal{X}$. and $B = max||g(x)||_2$ is the largest $l_2$ norm that $g(x)$ can achieve. 

The expectation of steps ($E_{SGD}$) needed by a SGD learning algorithm to learn $f$ within the error rate of $\epsilon$ is $\mathbb{E}_{SGD} = \frac{B^2L^2}{\epsilon^2}$, where $L$ is the Lipschitz constant of $f(x)$, i.e., $L=\sup\{L(f,\mathcal{X}_{x, \infty}), x \in \mathcal{X}\}$. 

Similarly, the expected steps ($E_{PGD}$) needed by a PGD learning algorithm to learn $f$ within the error rate of $\epsilon$ is $\mathbb{E}_{PGD} = \frac{L^2}{\alpha\epsilon}$, where $L$ is the Lipschitz constant of $f(x)$, and $\alpha$ is the step size. 

Finally, the expectation of steps ($E_{AGD}$) needed by a AGD learning algorithm to learn $f$ within the error rate of $\epsilon$ is $\mathbb{E}_{AGD} = R \sqrt{\frac{\beta}{\varepsilon}}$, where $\beta$ is the smoothness of $f(x)$.

\end{lemmabold}

Combining Lemma~\ref{Lemma:borrowed_SGD convergence} and Theorem~\ref{thm:trojan_increaseing_rate_function_lipschitz}, we conclude that the convergence of the gradient-based optimization is faster on the target function with the lower Lipschitz constant, which indicates gradient-based trigger inversion algorithms perform better on the triggers with higher robustness because the local Lipschitz constant around these triggers is lower. Note that here we utilize a convex relaxation to approximate the loss function around the trigger area. As a convex function, as long as the step size is proper, the optimizer could always converge to the global minimum (trigger), and techniques such as second-order optimizer or momentum could boost the convergence speed. However, in the analysis of the next two cases, we consider the non-convex case, in which we show that the second-order optimizer or optimizer utilizing momentum could not make it the optimizer easier to find the trigger. Furthermore, we provide an empirical result of the effectiveness of trigger inversion while using different types of optimizers such as second-order optimizer (AdaHessian\cite{adahessian}), optimizer utilizing momentum (Adam\cite{adam}) and SGD. The result in 13.7 of the online document~\cite{online_document} shows that the optimizer that utilizes momentum, such as Adam, is comparable with SGD. Second-order optimizer, such as AdaHessian, has relatively low performance while optimizing the trigger inversion. \cite{pixelbackdoor,abs,k-arm}  



Next, we study the gradient-based optimization of a non-convex function, starting from a one-dimensional function. Here, we consider the target function as a piece-wise linear function, representing a neural network using the activation function such as ReLU. %Theorem If we assume the trigger is the global optimal (high confidence trigger) in the loss function, informally, 
Theorem \ref{thm:MC_proof} shows the positive relationship between the robustness of a trigger (as the global optimum of the target function) and the probability that the gradient-based optimizer converges to the trigger.


\begin{theorembold}
\label{thm:MC_proof}
Given a piece-wise linear function $\ell(\cdot): [a,b] \rightarrow [0,1] $ with global optimum on a convex hull, after $n$ iterations, a gradient-based optimizer starting from a random initialization converges to the optimum with the probability:
\begin{equation}
1- B_1^{-1}(b-a)^{-1}(4-B_1B_2)^n(1-B_1B_2)]
\end{equation}

\end{theorembold}
\noindent where $B_1>0$ is a component indicating the area under the desired convex hull and $B_2>0$ is a component indicating the likelihood of the linear pieces outside the convex hull jumping into the convex hull during a gradient-based iteration (For details, see the proof of Theorem~\ref{thm:MC_proof} in 13.5 of the online document\cite{online_document}.)

Notably, in the gradient-based optimization for trigger inversion, the optima represent the desirable trigger-inserted points, and thus the size of the convex hull is positively correlated with the robustness of the trigger. As a result, the gradient-based trigger inversion has a higher probability of identifying the trigger when the trigger is more robust. 


Finally, we consider the target function as high-dimensional non-convex but satisfies the proximal-PL condition~\cite{PL_condition}, which is often considered in the theoretical analysis of neural networks. Formally, the proximal-PL condition is defined below.

\begin{definitionbold} [Proximal-PL condition]
We consider the optimization problem in the form:
\begin{equation}\label{formula:problem_proximal-PL}
    \underset{x \in \mathbb{R}^d}{\operatorname{argmin}} F(x)=f(x)+g(x),
\end{equation}
\noindent where $f$ is a differentiable function with an $L$-Lipschitz continuous gradient and $g$ is a simple but potentially non-smooth convex function \footnote{Typical examples of the simple function $g$ include a scaled $\ell_1$-norm of the parameter vectors (the size of the trigger), $g(x)=\lambda\|x\|_1$, and indicator functions that are zero if $x$ lies in a simple convex set, and are infinity otherwise.}. To analyze the proximal-gradient algorithms (i.e., a more general form of the Projected Gradient Descent (PGD)), a natural %(though not particularly intuitive) 
generalization of the PL inequality is that there exists $\mu>0$ satisfying:

\begin{equation}\label{formula:proximal-PL}
    \frac{1}{2} \mathcal{D}_g(x, L) \geq \mu\left(F(x)-F^*\right)
\end{equation}
where
\begin{equation*}
\scriptstyle
\mathcal{D}_g(x, \alpha) \equiv -2 \alpha \min _y\left[\langle\nabla f(x), y-x\rangle+\frac{\alpha}{2}\|y-x\|^2+g(y)-g(x)\right] .    
\end{equation*}
\end{definitionbold}

%We call this the proximal-PL condition. Below is the 
Theorem \ref{thm:PL_condition} from \cite{PL_condition} showed that the proximal-PL condition is sufficient for the proximal-gradient method to achieve a global linear convergence rate.

\begin{theorembold}\label{thm:PL_condition}
Consider the optimization problem in Eq.~\ref{formula:problem_proximal-PL}, where $f$ has an L-Lipschitz continuous gradient (Eq.~\ref{formula:proximal-PL}), $F$ has a non-empty solution set $\mathcal{X}^*, g$ is convex, and $F$ satisfies the proximal-PL inequality. Then the proximal gradient method with a step size of $1 / L$ converges linearly to the optimal value $F^*$:
\begin{equation}\label{eq: PL convergence rate}
    F\left(x_k\right)-F^* \leq\left(1-\frac{\mu}{L}\right)^k\left[F\left(x_0\right)-F^*\right\rceil
\end{equation}

\end{theorembold}

Theorem \ref{thm:PL_condition} also indicates a negative relationship between the Lipschitz constant ($L$) of the target function and the convergence rate to the local optimum (trigger) (i.e., the difference of the target function values between the optimal point and the actual trigger-inserted point). Previous research~\cite{cartis2018worst} showed that the second-order optimizer has exactly the same lower bound of convergence rate as the first-order optimizer under the PL condition. Many existing studies \cite{yang2020adversarial,terjek2019adversarial,krishnan2020lipschitz} showed that in neural networks, the lower Lipschitz constant implies the higher robustness of the model. Therefore, combining with Theorem~\ref{thm:PL_condition}, we conclude that the gradient-based trigger inversion methods perform well on the triggers with high robustness.  

\subsection{Why Inversion Fails under \ourmethod{}} \label{subsec: why Grasp can render}

%\subsection{Why \ourmethod{} can render trigger inversion ineffective} \label{subsec: why Grasp can render}

%\vspace{2pt}\noindent\textbf{Local Lipschitz enhancement}. 
Now we are ready to analyze the local Lipschitz constant around the trigger-inserted samples, in particular how it is influenced by the noise level (measured by the parameter $c$; see Theorem \ref{thm:trojan_increaseing_rate_function_lipschitz}) in the \ourmethod{} algorithm. Specifically, Theorem~\ref{thm1a} shows that when each of the two typical noise distributions is used, the \ourmethod{}-poisoned model will have greater local Lipschitz constant around $x$ than the model under the data poisoning attack without using \ourmethod{}, for example by BadNet\cite{badnet}.

Formally, consider a single case in \ourmethod{} data poisoning: a trigger $(\boldsymbol{M},\boldsymbol{\Delta})$ is injected into a single normal data point $(x,y)$, resulting in the trigger-inserted data point $(x',y_t)$, where $x' = A(x,\boldsymbol{M},\boldsymbol{\Delta})$. Let $(x^*,y)$ be the trigger-inserted data point with noise $\epsilon$ added on the trigger part, where $x^* = A(x,\boldsymbol{M},\boldsymbol{\Delta}) + c \cdot \epsilon \cdot \boldsymbol{M} $. Let $f$ be the \ourmethod{}-poisoned classification model, which we assume is astute at $(x,y)$, $(x^*,y)$ and $(x',y_t)$.

\begin{theorembold}
\label{thm1a}
If the noise $\epsilon \sim \mathcal{N}(0,1)$ (i.e., the white noise), and $c < \|x'-x\|_2 \cdot \frac{\Gamma\left(\frac{|m^*|}{2}\right)}{\sqrt{2} \Gamma\left(\frac{|m^*|+1}{2}\right)}$, where $|m^*|$ is the $l_1$ norm (i.e., the size) of the trigger, $\Gamma$ is the Euler’s gamma function. A model attacked by a backdoor attack and enhanced by \ourmethod{} using the training data points $(x,y),(x',y_t)$ and $(x^*,y)$ has a greater local Lipschitz constant around $x$ than the model backdoored by the same attack without the enhancement by \ourmethod{} using the training data points $(x,y),(x',y_t)$.

Similarly, if $\epsilon \sim uniform(-1,1)$, and $c < \|x'-x\|_2$,
the \ourmethod{}-enhanced model has greater local Lipschitz constant around $x$ than the model without the enhancement.


\end{theorembold}

The proof of Theorem~\ref{thm1a} is given in 13.6 of the online document\cite{online_document}. The theorem 
indicates that if the level of the noise used in \ourmethod{} is bounded by the $l_2$-distance between the normal data point $x$ and the trigger-inserted point $x'$, 
the \ourmethod{}-poisoned model will have a greater local Lipschitz constant, or intuitively, a steeper output around $x'$ compared with the model poisoned by existing backdoor attacks like BadNet. Combining Theorem~\ref{thm1a} with Theorems~\ref{thm:trojan_increaseing_rate_function_lipschitz},~\ref{thm:MC_proof} and~\ref{thm:PL_condition} in Section~\ref{subsec:3 condition}, we conclude that GRASP can render trigger inversion less effective.

%}


==> 6-evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Against Inversion-based Detection}
\label{sec:eval}
%\section{Backdoor Effectiveness Against Trigger Inversion Detection}

In this section, we evaluated the effectiveness of \ourmethod{} by comparing inversion-based backdoor defenses against different attacks before and after the enhancement by \ourmethod{}, respectively.


\subsection{Datasets and Settings}\label{subsec:Dataset}
\noindent\textbf{Datasets}. 
We analyzed backdoor attacks on the models trained using three public datasets: MNIST~\cite{lecun1998gradient}, CIFAR10~\cite{krizhevsky2009learning}, and GTSRB~\cite{Stallkamp2012}, as summarized by Table~\ref{tab:datasets}. Our experiments were conducted on a server with one AMD Ryzen 3980X 3.2 GHz 48-core processor and one NVIDIA RTX 3090 GPU.

\begin{table}[htp]
\centering
\captionsetup{font=small}
\begin{tabular}{l|c|c|c}
                      & MNIST & GTSRB & CIFAR10 \\ \hline
Training samples (\#) & 60,000  & 39,209  & 50,000  \\ 
Testing samples (\#)  & 10,000  & 12,630  & 10,000  \\ 
\end{tabular}
\caption{Datasets statistics}
\label{tab:datasets}
\vspace{-2mm}
\end{table}

\noindent\textbf{Backdoor attacks}. 
We considered seven existing backdoor attacks: BadNet~\cite{badnet}, LSBA~\cite{lsba}, Composite~\cite{composite}, clean label~\cite{latent}, DEFEAT~\cite{defeat}, IMC~\cite{IMC} and adaptive-blend~\cite{adaptive-blend}. Those backdoor attacks fall into four general categories: patch trigger, clean label, imperceptible, and latent space inseparable. For each attack, we generate and evaluate 24 backdoored models: for each of the three different datasets (MNIST, CIFAR-10, and GTSRB), we generate two models using each of four different neural network structures (VGG-16, ResNet-101, ShuffleNet, and ResNet18, respectively).



\vspace{3pt}\noindent$\bullet$\textit{ Patch trigger}. The patch triggers usually utilize a small pattern as the trigger for the backdoor attack. We select BadNet~\cite{badnet}, LSBA~\cite{lsba}, and Composite~\cite{composite} in this category and used two patterns (as shown in the 13.8 of the online document~\cite{online_document}) as the patch trigger in the backdoor attack.

\vspace{3pt}\noindent$\bullet$\textit{ Clean label}. The clean-label backdoor attacks contaminate the training dataset with the clean-label data. We select Latent~\cite{latent} to represent the attacks in this category.

\vspace{3pt}\noindent$\bullet$\textit{ Imperceptible}. An imperceptible backdoor attack aims to design a backdoor trigger that can evade human inspection. Most of these attacks enhance the backdoor stealthiness through universal adversarial perturbation (UAP). We select DEFEAT~\cite{defeat} and IMC~\cite{IMC} in this category in our experiments.

\vspace{3pt}\noindent$\bullet$\textit{ Latent space inseparable}. A latent space inseparable backdoor attack aims to design a backdoor trigger so that in the latent space of the target model, the trigger-inserted samples are close to the clean samples in the target class. We select Adaptive-Blend~\cite{adaptive-blend} in this category in our experiment.

\vspace{3pt}\noindent$\bullet$\textit{ Attack parameters}. We inserted 3000, 2352, and 3000 poisoning data samples (i.e., 6\% poisoning rate) into the training datasets of CIFAR-10, MNIST, and GTSRB, respectively. Following original papers, the trigger in IMC was synthesized~\cite{IMC}, and the trigger in Latent was randomly initialized~\cite{latent}.
% \ignore{So the total numbers of training samples in these datasets were 53,000, 41,561, and 53,000, respectively.}

% \ignore{\vspace{3pt}\noindent$\bullet$\textit{ BadNet attack}. We inserted  3000, 2352, and 3000 poisoning data samples (6\% of the entire set) into the training datasets of CIFAR-10, MNIST and GTSRB, respectively. So the total numbers of training samples in these datasets were 53,000, 41,561, and 53,000, respectively.}

\vspace{3pt}\noindent$\bullet$\textit{ \ourmethod{}}. For each attack mentioned above, we combine them with \ourmethod{} by algorithm~\ref{alg:one}. More specifically, we inserted 6\% poisoning data to the training datasets, among which 3\% are trigger-inserted samples, and the other 3\% are the same trigger-inserted samples with noises and source-class labels (Algorithm~\ref{alg:one}). 



\vspace{3pt}\noindent\textbf{Trigger inversion}. 
We implemented and tested four backdoor countermeasures based upon trigger inversion: Neural Cleanse~\cite{NC}, TABOR~\cite{tabor}, K-arm~\cite{k-arm}, and Pixel~\cite{pixelbackdoor}. In our experiments, we utilized 10\% of the training data and the default hyper-parameters provided in the original papers for trigger reconstruction. 



\subsection{Putative Trigger Effectiveness}\label{subsec: Trigger accuracy}

% Backdoor detection often serves as the first step in backdoor defense, followed by backdoor mitigation or unlearning to remove the backdoor from an infected model. These downstream mitigation approaches all depend on the triggers reconstructed by the trigger inversion algorithms, whose accuracy may not be easily measured: 
Existing methods measure the effectiveness of trigger inversion by computing the similarity between the reconstructed and real triggers, e.g., based on $l_1$ distance, which is insufficient since a similar pattern may not have a similar backdoor effect (i.e., ASR). We propose a set of metrics to measure trigger accuracy. Below we present our experimental results on the effectiveness of backdoor detection by four trigger inversion algorithms: (NC~\cite{NC}, TABOR~\cite{tabor}, Pixel~\cite{pixelbackdoor}, and K-arm~\cite{k-arm}), by comparing the effectiveness of the backdoor attacks before and after the enhancement by \ourmethod{}. More specifically, after the trigger is generated by each backdoor attack method, we use \ourmethod{} to enhance this trigger as described in section~\ref{subsec: Gradient Shaping}. Here, we append a symbol ``*" to the name of each backdoor attack to indicate the respective attack enhanced by \ourmethod{}. For example, ``BadNet*" indicates BadNet enhanced by \ourmethod{}. 

\vspace{3pt}\noindent\textbf{Metrics}. 
In our experimental study, we utilize four quantitative metrics to measure the effectiveness of a backdoor in evading a gradient-based inversion algorithm (for reconstructing a trigger $(\boldsymbol{\Delta}, \boldsymbol{M})$ in a model $f$):  

\vspace{2pt}\noindent$\bullet$~$\epsilon_1$: The difference between the real trigger's ASR on the backdoored model and that on the ``sanitized'' model retrained to unlearn the reconstructed trigger: that is, $\epsilon_1 = |ASR_{unlearn}-ASR|$. A smaller difference indicates that the reconstructed trigger is less accurate, thus, unlearning is less effective.

\vspace{2pt}\noindent$\bullet$~$\epsilon_2$: The Jaccard distance between the trigger mask of the reconstructed trigger $M'$ and of the real trigger $M$ can be calculated as $J(M',M) = \frac{|M' \cap M|}{|M'|+|M|-|M' \cap M|}$.


\vspace{2pt}\noindent$\bullet$~$\epsilon_3$: The ASR of the reconstructed trigger $(\boldsymbol{M'},\boldsymbol{\Delta'})$ on a clean model $f^*$: $\epsilon_4 = ASR_{f^*}'$. A large $ASR_{f^*}'$ indicates that the reconstructed trigger is likely a natural trigger~\cite{liu2020reflection}, not the real one meant to be recovered.

\vspace{2pt}\noindent $\bullet$~$\epsilon_4$: $AUC$ score of backdoor detection. The trigger inversion methods often use the $l_0$ norm of the reconstructed trigger as the measurement to distinguish backdoored models from benign models: the lower of the $l_0$ norm, the more probable the model has been backdoored.

% $\bullet$~$l_1$ norm: The $l_1$ norm of the reconstructed trigger mask, which is supposed to be small for a real trigger~\cite{NC}.
%This norm suppose to be small, as the real triggers we injected all have small norms. 
%\end{itemize}

Notably, for a trigger inversion algorithm with ideal performance,
  $\epsilon_3$ is anticipated to be close to 0, while $\epsilon_1$,$\epsilon_2$ and $\epsilon_4$ are anticipated to be close to 1. 

\vspace{3pt}\noindent\textbf{Experimental results}. Here we present our results as measured by the aforementioned metrics. Due to the space limit, we defer our complete experimental results to Table~\ref{tab:trigger_accuracy_1} in Appendix and only report representative results ($\epsilon_4$) in this section.

\vspace{2pt}\noindent$\bullet$\textit{~$\epsilon_1$: effectiveness of unlearning}.
The reconstructed trigger can be used for backdoor unlearning~\cite{NC,tabor,k-arm}.  
After we reconstructed the trigger for a given backdoored model during the unlearning procedure, we first built an unlearning dataset, including randomly selected 10\% of the training data (6,000 in MNIST, 5,000 in CIFAR-10, and 3,920 in GTSRB). Then, we added the reconstructed trigger onto 10\% of the unlearning dataset (600 in MNIST, 500 in CIFAR-10, and 392 in GTSRB) while keeping their class labels intact (the original source class). After that, we fine-tuned the model on this unlearning dataset. We used SGD as the optimizer in the experiment and set the learning rate = $0.01$ and momentum = $0.9$. As shown in Table~\ref{tab:trigger_accuracy_1}, after unlearning with the reconstructed trigger by various trigger inversion algorithms, most models poisoned by the attack enhanced by \ourmethod{} still preserve much higher ASRs (almost identical to those before unlearning), so that the \ourmethod{}-enhanced attacks achieve lower $\epsilon_1$ than respective backdoor attack. Table\ref{tab:trigger_accuracy_1} shows that on  CIFAR-10, BadNet achieves the worse performance against the trigger inversion defense of Tabor ($\epsilon_1 = 97.5\%$), which is significantly enhanced by \ourmethod{} ($\epsilon_1 = 1.5\%$). Among other attacks, LSBA* has the best performance under pixel as 0.6\%.

\vspace{2pt}\noindent$\bullet$\textit{~$\epsilon_2$: distance between trigger masks}. We observed that the reconstructed triggers from the models poisoned by \ourmethod{}-enhanced attacks have very low similarity with the real triggers (i.e., the overlap between the real and the reconstructed triggers are less than 20\%). By comparison, the reconstructed triggers from the models under the backdoor attacks without \ourmethod{} enhancement overlap with the real triggers by about 10\% - 60\%. On CIFAR-10, when enhanced by \ourmethod{}, DEFEAT* has worse performance against pixel ($\epsilon_2 = 0.13$). While BadNet* has the best performance against NC ( $\epsilon_2 = 0.00$) (Table~\ref{tab:trigger_accuracy_1}).


\vspace{3pt}\noindent$\bullet$\textit{~$\epsilon_3$: $ASR$ of the reconstructed triggers on a clean model}. 

We also computed $\epsilon_3$, the ASR of the reconstructed triggers from the poisoned models %$(\boldsymbol{\Delta_t},\boldsymbol{M_t})$ 
on a clean model for the same task. In our experiment, we used CIFAR-10, MNIST, and GTSRB as the clean datasets to train the clean models. After a trigger is reconstructed from a poisoned model, we randomly select 500 images from the source class of the clean dataset and insert the trigger on them. The ASR was then measured on this set of trigger-inserted samples on the clean model. As shown in Table~\ref{tab:trigger_accuracy_1}, %third part of Table~\ref{tab: trigger accuracy}, 
the reconstructed triggers from the models poisoned by \ourmethod{}-enhanced attacks have a relatively high ASRs on the clean model, almost comparable with their ASRs on the poisoned models, whereas the reconstructed triggers from the models poisoned by the attack without \ourmethod{} enhancement have much lower ASRs. This indicates that any useful trigger recovered from the models poisoned by \ourmethod{}-enhanced attacks are likely to be a natural trigger  introduced by the legitimate learning process that has nothing to do with the injected triggers. 
%indicating that for the models poisoned by \ourmethod{}, the reconstructed triggers are in fact not the same as the real triggers. 
 On dataset CIFAR-10,  when enhanced by \ourmethod{}, LSBA* has worse performance against pixel ($\epsilon_3 = 42.1\%$) while Adaptive-Blend has the best performance against ($ \epsilon = 28.3\%$). 

\vspace{2pt}\noindent$\bullet$\textit{~$\epsilon_4$ AUC}.  
As mentioned earlier, our research shows that trigger inversion algorithms are unlikely to effectively reconstruct and remove the triggers injected by \ourmethod{}, even though they are largely successful on the triggers injected by existing backdoor attacks. 
In some cases, however, the backdoor defense methods just need to detect the infected models (and discard them afterward), even though they cannot accurately reconstruct the real trigger. 
Our research evaluated how successfully these trigger inversion methods can detect the models poisoned by \ourmethod{}-enhanced attacks. Specifically, we train 24 clean models; for each of the three different datasets (MNIST, CIFAR-10, and GTSRB), we generate two clean models using each of four different neural network structures (VGG-16, ResNet-101, ShuffleNet, and ResNet18, respectively) to analyze their detection accuracy. Similarly, we train 24 models for each attack on three datasets using four neural network structures. In our research, we measured the AUC score of NC, TABOR, K-arm, and Pixel on these 48 models (24 clean models and 24 backdoored models). As shown in Table~\ref{tab:trigger_AUC}, generally speaking, the AUC scores of different defense strategies from the models poisoned by different backdoor attacks with \ourmethod{} enhancement are significantly smaller than those from the models poisoned by the same attack without \ourmethod{} enhancement, which indicates the better effect of the \ourmethod{}-enhanced attacks to evade the detection by all tested triggers inversion algorithms. In particular, LSBA enhanced by \ourmethod{} successfully evades the detection by the trigger inversion algorithms with AUCs below 65\% for all of them. 










\vspace{-2.5mm}

\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{l|lllll|llll|llll}
\multicolumn{2}{l|}{}       & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{MNIST} & \multicolumn{4}{c}{GTSRB}\\
\multicolumn{2}{l|}{}       & NC  & Tabor  & K-arm  & Pixel & NC & Tabor & K-arm & Pixel & NC & Tabor & K-arm & Pixel \\ 

\hline
\multicolumn{13}{c}{$\epsilon_4$: AUC }\\
\hline 
\hline
%                                   CIFAR-10                                        MNIST                                          GTSRB      
%                                   & NC        & Tabor     & ABS       & Pixel     & NC       & Tabor     & ABS       & Pixel     & NC        & Tabor     & ABS       & Pixel \\ 
%Patch
\multicolumn{2}{l|}{BadNet}         & 79.1\%    & 83.5\%    & 84.6\%    & 92.3\%    & 77.9\%   & 81.6\%    & 83.2\%    & 89.7\%    & 79.9\%    & 82.0\%    & 85.1\%    & 89.6\%   \\
\multicolumn{2}{l|}{BadNet*}        & 54.2\%    & 55.3\%    & 59.2\%    & 79.4\%    & 53.3\%   & 54.3\%    & 59.9\%    & 83.4\%    & 53.4\%    & 56.2\%    & 58.2\%    & 81.3\%   \\
\multicolumn{2}{l|}{LSBA}           & 67.2\%    & 67.4\%    & 71.4\%    & 81.6\%    & 68.2\%   & 68.9\%    & 71.0\%    & 79.0\%    & 69.1\%    & 69.5\%    & 71.0\%    & 87.2\%   \\
\multicolumn{2}{l|}{LSBA*}          & 54.4\%    & 56.0\%    & 59.1\%    & 63.3\%    & 52.6\%   & 57.7\%    & 56.1\%    & 63.5\%    & 53.9\%    & 52.9\%    & 58.9\%    & 65.4\%   \\
\multicolumn{2}{l|}{Composite}      & 67.1\%    & 65.3\%    & 69.2\%    & 84.5\%    & 65.5\%   & 64.2\%    & 69.0\%    & 83.3\%    & 66.2\%    & 68.3\%    & 69.5\%    & 84.9\%   \\
\multicolumn{2}{l|}{Composite*}     & 53.2\%    & 59.3\%    & 61.4\%    & 72.4\%    & 53.1\%   & 52.0\%    & 59.3\%    & 71.1\%    & 55.3\%    & 53.1\%    & 59.1\%    & 72.1\%   \\
%Clean label
\multicolumn{2}{l|}{Latent}    & 78.5\%    & 76.3\%    & 79.5\%    & 87.4\%    & 80.1\%   & 79.5\%    & 81.6\%    & 89.1\%    & 76.3\%    & 79.3\%    & 76.1\%    & 85.8\%   \\
\multicolumn{2}{l|}{Latent*}   & 53.1\%    & 55.2\%    & 59.2\%    & 75.3\%    & 53.9\%   & 55.1\%    & 58.8\%    & 74.1\%    & 53.1\%    & 54.1\%    & 57.3\%    & 70.6\%   \\
%Imperceptible
\multicolumn{2}{l|}{DEFEAT}         & 64.5\%    & 63.9\%    & 77.5\%    & 69.3\%    & 67.3\%   & 69.0\%    & 80.2\%    & 71.5\%    & 64.2\%    & 68.1\%    & 79.4\%    & 66.1\%   \\
\multicolumn{2}{l|}{DEFEAT*}        & 59.5\%    & 59.4\%    & 72.4\%    & 62.1\%    & 58.7\%   & 58.2\%    & 71.1\%    & 59.4\%    & 59.1\%    & 58.2\%    & 71.2\%    & 62.3\%   \\
\multicolumn{2}{l|}{IMC}            & 68.3\%    & 65.0\%    & 76.1\%    & 79.5\%    & 67.3\%   & 69.0\%    & 77.4\%    & 79.5\%    & 70.1\%    & 72.3\%    & 76.1\%    & 77.0\%   \\
\multicolumn{2}{l|}{IMC*}           & 55.5\%    & 54.7\%    & 72.2\%    & 71.5\%    & 54.4\%   & 53.6\%    & 74.3\%    & 74.1\%    & 66.3\%    & 61.0\%    & 71.5\%    & 77.3\%   \\
%Latent space similarity
\multicolumn{2}{l|}{Adaptive-Blend} & 66.3\%    & 67.3\%    & 67.4\%    & 77.4\%    & 59.3\%   & 63.1\%    & 65.1\%    & 81.2\%    & 64.2\%    & 63.4\%    & 65.0\%    & 78.9\%   \\
\multicolumn{2}{l|}{Adaptive-Blend*}& 55.2\%    & 54.0\%    & 54.4\%    & 68.7\%    & 52.3\%   & 59.1\%    & 61.0\%    & 75.2\%    & 57.3\%    & 54.2\%    & 59.1\%    & 69.1\%   \\


\end{tabular}
\caption{The AUCs of backdoor detection by trigger inversion methods on the backdoored models poisoned by different backdoor attacks with and without the enhancement of \ourmethod{}. The attack with the \ourmethod{} enhancement is denoted by the symbol ``*" appended to the name of the respective attack.}
\label{tab:trigger_AUC}
\end{table*}

==> 7-Effectiveness-Against-Weight-Analysis.tex <==
\section{Against Weight Analysis Detection}

Weight Analysis aims to distinguish backdoor and benign models by analyzing the signals in model parameters. Specifically, the distinguishable signals within the parameters between the backdoor and benign model are extracted, often through training a classifier on parameters of sample models, and then utilized to predict whether any given model is backdoored~\cite{trojan_signiture}\cite{AC}\cite{du2019robust}. In this section, we present theoretical and experimental studies to show that backdoored models poisoned by a \ourmethod{}-enhanced attack are not further away from the benign models of the same primary task than the backdoored model poisoned by the same attack without \ourmethod{} enhancement.

Formally, given a training dataset $D$, and a backdoor attack, we train $t$ benign ML models $\{f_{\theta_{(i)}}| i \in \{1,2,...,t\}\}$ on $D$, and $t$ backdoored ML models $\{f_{\hat{\theta}_{(i)}}| i \in \{1,2,...,t\}\}$ on $D$ with the given backdoor attack.  $z(f_\theta(\cdot)):\mathcal{X}^m \rightarrow \mathcal{Y}$, where $\theta \in \mathbb{R}^K$ represent the set ($K$) parameters in the model $f_{\theta}$. A weight analysis methods then build a classifier $g(\cdot): \mathbb{R}^K \rightarrow [0,1]$, which is trained on the dataset $D_{\theta} = \{(\theta_{(1)},0), (\theta_{(2)},0),...,(\theta_{(t)},0) \} \cup \{(\hat{\theta}_{(1)},1), (\hat{\theta}_{(2)},1),...,(\hat{\theta}_{(t)},1) \}$ where the label $``0"$ indicates the parameters of benign models, and $``1”$ indicates the parameters of backdoored models. 



Next, we show why \ourmethod{} does not reduce the attack effectiveness to evade the weight analysis. Consider a neural network with any initialization $f_{\theta_0}$ is trained on the dataset $D_{benign}$, the backdoor dataset $D_{backdoor}$, and the \ourmethod{}-enhanced backdoor dataset $D_{GRASP}$, respectively. Specifically, we denote $D_{benign} = \{D_{ori}, D^*_{troj}, D^*_{Aug} \}$, $D_{backdoor} = \{D_{ori}, \hat{D}_{troj}, \hat{D}_{Aug} \}$, and $D_{GRASP} = \{D_{ori}, \hat{D}_{troj}, D^*_{Aug} \}$, where $D_{ori}$ is the legitimate training dataset used for training all three models, $\hat{D}_{troj}$ and $D^*_{troj}$ represent the set of trigger inserted samples labeled by the target and the source (legitimate) class, respectively, and $\hat{D}_{Aug}$ and $D^*_{Aug}$ represent the set of augmented samples (i.e., the trigger-inserted samples with added noise) labeled by the target and the source (legitimate) classes, respectively.


Theorem~\ref{thm:weight analysis} below indicates the models trained on $D_{GRASP}$ (enhanced by \ourmethod{}) are not easier to be distinguished by the weight analysis from the benign models (trained on $D_{benign}$) than the models trained on $D_{backdoor}$ (by the backdoor attack without \ourmethod{} enhancement).


\begin{theorembold}
\label{thm:weight analysis}
Consider a $L$ - layer neural network $f_{\theta}(\cdot): \mathcal{X}^m \rightarrow \bar{\mathcal{Y}}$. Given an input $x\in \mathcal{X}^m$, in the $l^{th}$ layer with $K_{(l)}$ neurons, where $1<l<L$, let $\phi(x)^{(l)}_{k}$ denote the output of the $k^{th}$ neuron before activation, and $\sigma (x)^{(l)}_{k}$ denote denote the output after activation. Let $\theta ^{(l)}_{(p,q)}$ denote the weight connecting $q^{th}$ neuron in the $(l-1)^{th}$ layer and $p^{th}$ neuron in the $l^{th}$ layer.

We assume:

\begin{equation}
 \sum\limits^{D_{ori}}_i \sigma(x_i)^{(l)}_k \cdot \sum\limits^{D_{troj}^*}_i \sigma(x_i)^{(l)}_k\cdot \sum\limits^{D_{Aug}^*}_k \sigma(x_i)^{(l)}_i \neq 0
\end{equation}

\noindent and the square loss function $C(\theta) = \frac{1}{2m} \sum\limits^n_i (f(x_i;\theta)-y_i)^2$
is used for training.
Then for any set of parameters $\theta$, the gradient of the loss function w.r.t any parameter $\theta^{(l)}_{(p,q)}$ in the model $f_{\theta}$ on the three datasets satisfy:

\begin{equation}\label{eq:weight analysis}
\scriptsize\mathop{\nabla}\limits_{D_{benign}}\theta^{(l)}_{(p,q)} - \mathop{\nabla}\limits_{D_{backdoor}}\theta^{(l)}_{(p,q)}  >   \mathop{\nabla}\limits_{D_{benign}}\theta^{(l)}_{(p,q)} - \mathop{\nabla}\limits_{D_{GRASP}}\theta^{(l)}_{(p,q)}
\end{equation}

\end{theorembold}

The proof of Theorem~\ref{thm:weight analysis} is given in the Appendix. This theorem shows the difference of gradient on the parameters between the backdoored models poisoned by a \ourmethod{}-enhanced attack and the benign models is always smaller than the difference between the backdoored models poisoned by the same attack without \ourmethod{} enhancement, which implies it is not easier to distinguish the \ourmethod{} poisoned models from benign models than to distinguish the backdoored models without \ourmethod{} enhancement from the benign models.

We then evaluated the effectiveness of \ourmethod{} against the weight analysis-based backdoor detection, which has been adopted by some teams and performed well in some cases in recent backdoor competitions~\cite{trojai, NIPS_competation}. Here we selected Trojan Signature (TS)\cite{trojan_signiture},  MNTD\cite{MNTD}, Activation Clustering (AC)~\cite{clustering} and ABS~\cite{abs}, the representative methods based on weight analysis. We computed their AUCs on 20 models using VGG16, including ten clean models and ten backdoored models, respectively, trained on each of the three datasets (CIFA-10, MNIST, and GTSRB). The backdoored models were poisoned by the three backdoor attacks with or without the \ourmethod{} enhancement, respectively. Here, the three attacks were selected because they were shown to be effective against the weight analysis-based backdoor defense. Due to the space limit, we only present the most important results in Table \ref{tab: weight analysis results}, the entire results are presented in Table~\ref{tab:weight analysis AUC entire}. In general, the detection ability (AUC) by the weight analysis methods is lower or comparable on the three attacks when they are enhanced by \ourmethod{}, indicating \ourmethod{} enhancement does not reduce the effectiveness of these attacks against the weight analysis backdoor defense.


\begin{table}[htp]
\centering
\footnotesize
\captionsetup{font=small}
\begin{tabular}{ll|l|l|l}
\multicolumn{2}{l|}{}                                                       & CIFAR-10    & MNIST    & GTSRB         \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{ABS}}                 & DFST             &  67.4\%    &  65.0\%  &  68.4\%       \\
\multicolumn{1}{l}{}                                     & DFST*            &  63.1\%    &  62.7\%  &  62.0\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{AC}}                  & AB               &  68.4\%    &  69.1\%  &  67.1\%       \\
\multicolumn{1}{l}{}                                     & AB*              &  57.2\%    &  59.0\%  &  60.3\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{TS}}                  & DEFEAT           &  68.9\%    &  67.3\%  &  67.0\%       \\
\multicolumn{1}{l}{}                                     & DEFEAT*          &  60.5\%    &  68.0\%  &  70.2\%        \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{MNTD}}                & DEFEAT           &  69.2\%    &  73.1\%  &  71.3\%       \\
\multicolumn{1}{l}{}                                     & DEFEAT*          &  66.0\%    &  72.9\%  &  71.7\%        \\ 
\end{tabular}
\caption{The AUCs of weight analysis-based backdoor detection methods on the benign and backdoored models poisoned by DFST, AB, and DEFEAT with and without \ourmethod{} enhancement.}
\label{tab: weight analysis results}
\vspace{-5mm}
\end{table}



==> 8-other.tex <==
\section{Resilience to Backdoor Mitigation}
\label{sec:other}

In this section, we evaluated the resilience of \ourmethod{} to the backdoor defense methods without using backdoor detection. In our experiments, we considered five types of backdoor defenses (mitigation or unlearning) as summarized in \cite{backdoorsurvey}: Preprocessing-based Defenses, Model Reconstruction, Poison Suppression, and Certified Backdoor Defense, which are not based on backdoor detection, such as trigger inversion or weight analysis. We selected a total of six typical defense methods across these four types: DeepSweep (DS)\cite{zeng2020deepsweep}, Fine-pruning (FP)~\cite{fine-purning}, NAD~\cite{NAD},  GangSweep (GS)~\cite{zhu2020gangsweep}, DBD~\cite{du2019robust}, RAB~\cite{rab}, and compared their performance on defending the selected backdoor attacks before and after the \ourmethod{} enhancement.

We measured the ASRs of backdoors after the backdoor mitigation on the models (VGG16) poisoned by the selected backdoor attacks with or without the \ourmethod{} enhancement, respectively. Here, for each defense method, we selected a backdoor attack that has been shown to effectively evade the respective defense in previous studies to demonstrate the enhancement by \ourmethod{} does not reduce its effectiveness to evade the respective defense methods. 

We summarize the results from both experiments in Table~\ref{tab: Other defense}. Except for special notes, all backdoored models before mitigation achieve an ASR above 95\%. Here, the notations are the same as used in Section \ref{sec:eval}: a symbol ``*" is appended to the name of the backdoor attack to indicate the respective attack enhanced by \ourmethod{}. Below, we discuss the results of different defense methods in detail.

\begin{table}[htp]
\centering
\footnotesize
\captionsetup{font=small}
\begin{tabular}{ll|l|l|l}
\multicolumn{2}{l|}{}                                                       & CIFAR-10    & MNIST    & GTSRB         \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{DS}}                  & HaS-Net          &  67.2\%    &  68.9\%  &  63.2\%       \\
\multicolumn{1}{l}{}                                     & HaS-Net*         &  65.1\%    &  68.3\%  &  64.2\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{FP}}                  & DEFEAT           &  81.4\%    &  87.6\%  &  86.4\%       \\
\multicolumn{1}{l}{}                                     & DEFEAT*          &  83.2\%    &  88.0\%  &  84.2\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{NAD}}                 & DEFEAT           &  79.2\%    &  81.1\%  &  82.5\%       \\
\multicolumn{1}{l}{}                                     & DEFEAT*          &  79.6\%    &  80.3\%  &  78.3\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{DBD}}                 & IMC              &  54.2\%    &  59.7\%  &  55.0\%       \\
\multicolumn{1}{l}{}                                     & IMC*             &  63.5\%    &  64.0\%  &  62.6\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{GS}}                  & AB               &  64.9\%    &  59.3\%  &  61.0\%       \\
\multicolumn{1}{l}{}                                     & AB*              &  65.4\%    &  63.2\%  &  61.4\%       \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{RAB}}                 & DFST             &  95.3\%    &  94.1\%  &  94.2\%       \\
\multicolumn{1}{l}{}                                     & DFST*            &  94.6\%    &  91.2\%  &  90.4\%       \\
\end{tabular}
\caption{The ASRs of the backdoored models after the mitigation by the backdoor mitigation methods, Note that the high ASR indicates that a backdoor attack is more resilient to the respective defense method. Here, all models are trained using three different datasets, and the backdoored models are infected by different attacks with and without the enhancement of  \ourmethod{}. (The attacks enhanced by \ourmethod{} is denoted by ``*").}
\label{tab: Other defense}
\vspace{-5mm}
\end{table}

\vspace{3pt}\noindent\textbf{Preprocessing-based Defenses}. Preprocessing-based defenses aim to remove the putative poison samples in the training dataset. DeepSweep (DS)~\cite{zeng2020deepsweep} is selected as the representative in this category. We tested the average ASR against the models infected by HaS-Net~\cite{low-conf}, which is a low-confidence backdoor attack. The ASRs of the models poisoned by the \ourmethod{}-enhanced HaS-Net attack (HaS-Net*) after the DeepSweep mitigation is comparable with those on the model poisoned by the HaS-Net attack (Table~\ref{tab: Other defense}), which indicates \ourmethod{} enhancement did not make the Has-Net backdoored models more easily mitigated by the DeepSweep. 


\vspace{3pt}\noindent\textbf{Model Reconstruction}. 
Fine-pruning~\cite{fine-purning} and NAD~\cite{NAD} are two typical model reconstruction methods to remove the backdoor.  
We conducted an experiment to compare the performance of Fine-pruning and NAD to defend against DEFEAT~\cite{defeat} with or without \ourmethod{} enhancement (DEFEAT or DEFEAT*). Table~\ref{tab: Other defense} shows the ASRs of the injected trigger after fine-pruning and NAD on the respective backdoored models. Note that the model reconstruction methods typically strike a trade-off between the accuracy of the primary task (ACC) and ASR. In our experiment, to keep the fidelity of the mitigation, we control the mitigation procedure such that the ACC does not  decrease by more than 5\%. We use 10\% of clean training data for mitigation, and for fine-pruning, we set 10\% activation pruning.   

Overall, the ASRs of the Fine-prune and NAD on the DEFEAT* attacked models are comparable with the DEFEAT attacked models, indicating the DEFEAT attack with and without \ourmethod{} enhancement are similarly effective against the Fine-pruning and NAD mitigation methods.

\vspace{3pt}\noindent\textbf{Non-Gradient Based Trigger Synthesis}.
Gangsweep~\cite{zhu2020gangsweep} is a non-gradient-based trigger synthesis defense that used the reconstructed trigger for backdoor mitigation. We performed an experimental study to confirm Adaptive-blend enhanced by \ourmethod{} (Adaptive-Blend*) does not generate the backdoors that can be easily mitigated by Gangsweep (GS). Table~\ref{tab: Other defense} shows the ASRs after the mitigating of Gangsweep on the backdoored models created by using Adaptive-Blend (AB) with or without \ourmethod{} enhancement. The ASR on the model attacked by \ourmethod{}-enhanced AB (AB*) is comparable (for the GTSRB dataset) or lower (for the CIFAR and MNIST dataset) than the ASRs on the models attacked by AB, indicating \ourmethod{} enhancement does not make the attack more easily to be mitigated by the Gangsweep.




\vspace{3pt}\noindent\textbf{Poison Suppression}.
For poison suppression defense, most methods (e.g., DBD~\cite{DBD}) learn a backbone of a DNN model via self-supervised learning based on training samples without their labels to capture those suspicious training data during the training process. 
We tested the performance of DBD~\cite{DBD} defense against models attacked by IMC\cite{IMC} with and without \ourmethod{} enhancement. As shown in Table \ref{tab: Other defense}, the ASR of the DBD in the IMC* attacked models are higher than the IMC attacked models, indicating \ourmethod{} enhancement does not make the attack more easily to be mitigated by the DBD.

\vspace{3pt}\noindent\textbf{Certified Backdoor Defense}.
RAB~\cite{rab} is a certified defense method that aims to eliminate the backdoor in the target model. We performed an experimental study to confirm \ourmethod{} enhancement does not generate the backdoor that is more easily mitigated by RAB.  Table\ref{tab: Other defense} shows the ASR of the injected trigger after RAB on the same models which attacked by DFST\cite{DFST} and DFST enhanced by \ourmethod{} (DFST*).
The ASR on DFST* is comparable to that on the DFST attacked models (GTSRB has the most significant difference, which DFST* is 3.8\% lower than DFST), indicating combing \ourmethod{} backdoored models are not easier to mitigate by the RAB than the model infected by DFST. 




In summary, we find that for the attacks that effectively evade backdoor mitigation, the \ourmethod{}enhancement  will not make the mitigation less effective. This means that \ourmethod{} enhancement can effectively fend off the existing backdoor defenses even though it is designed for evading trigger mitigation. For some mitigation methods like DBD, the IMC attack, the \ourmethod{} enhancement in fact increases their effectiveness.



% is less vulnerable to detection by all types of backdoor detection techniques compared with BadNet. It means that \ourmethod{} can fend off the existing backdoor defenses more effectively even given the fact that it is designed specifically for defeating trigger inversion.  
% Also it is important to note that these approaches, even when they appear to be effective on \ourmethod{}, work under different threat models than trigger-inversion based solutions and require more resources, particularly clean samples and poisoned samples, to detect backdoor triggers. For example, Activation clustering, Gangsweep, Anomalous Logits, and RAB require trigger-carrying samples or even the whole training dataset, and Fine-pruning requires a large amount of clean data (at least 10\% of the training data). With the help of these extra resources, they could perform better on \ourmethod{} than trigger inversion. Also for ABS, we can see that the detection accuracy on \ourmethod{} is significantly lower than on BadNet, possibly due to the fact that it includes a trigger inversion component. 


==> 9-mitigation-and-limitaion.tex <==
\section{Mitigation and Limitation}
\label{sec:discussion}
%Limitaion:***
%Our method is designed to evade trigger inversion algorithms, 
%For 
%
%Discussion:

%There is one question may concern about. 
\ourmethod{} can successfully increase the change rate around the trigger-inserted inputs, effectively reducing the trigger robustness of these inputs. 
Note that the trigger robustness should not be reduced to be lower than the obstructed robustness since otherwise, the backdoor attack may be defended by a straightforward strategy during inference: one can add the noise at the level above the robust radius of the backdoor task but below the robust radius of the primary task into each input; as such, the trigger-inserted inputs will not be predicted as the target class while the prediction of the benign input will not be changed, indicating the backdoor is removed without affecting the primary task.  
In practice, we found it is easy to reduce the  trigger robustness while keeping it above the obstructed robustness, as we observed that in the BadNet backdoor attack, the trigger robustness is always much greater than obstructed robustness (as shown in fig.~\ref{fig:rob_hist}).  
Therefore, it is always possible for \ourmethod{} to generate backdoors more effectively to evade the trigger-inversion algorithms while not affecting the performance of the primary task.



%\vspace{3pt}\noindent$\bullet$\textit{~ Limitation: Low confidence trigger}. 
In Section~\ref{sec:GRASP}, we assume the model will always give approximately 100\% confident prediction (as the target class) on all trigger-inserted inputs. In practice, when this assumption does not hold, for example, in~\cite{ali2020has}, where a low confidence backdoor is injected into the model by manipulating the logits of the poisoning data, the change rate around a perfect trigger may not be very large. Specifically, %when we have a low confidence trigger, 
the trigger-inserted inputs may be predicted as the target class with the lowest confidence in the backdoored model, which turns out to be a perfect trigger without any constraints on the local Lipschitz constant. For such backdoors, \ourmethod{} cannot further enhance their stealthiness.
